On the Parameterized Approximability of Contraction to Classes of Chordal Graphs

A graph operation that {\em contracts edges} is one of the fundamental operations in the theory of graph minors. Parameterized Complexity of editing to a family of graphs by contracting $k$ edges has recently gained substantial scientific attention, and several new results have been obtained. Some important families of graphs, namely the subfamilies of chordal graphs, in the context of edge contractions, have proven to be significantly difficult than one might expect. In this paper, we study the \textsc{$\cal F$-Contraction} problem, where $\cal F$ is a subfamily of chordal graphs, in the realm of parameterized approximation. Formally, given a graph $G$ and an integer $k$, \textsc{ $\cal F$-Contraction} asks whether there exists $X \subseteq E(G)$ such that $G/X \in \cal F$ and $|X| \leq k$. Here, $G/X$ is the graph obtained from $G$ by contracting edges in $X$. We obtain the following results for the \textsc{ $\cal F$-Contraction} problem. $(1)$ We show that \textsc{Clique Contraction} admits a polynomial-size approximate kernelization scheme (\textsf{PSAKS}). $(2)$ We give a $(2+\epsilon)$-approximate polynomial kernel for \textsc{Split Contraction} (which also implies a factor $(2+\epsilon)$-\FPT-approximation algorithm for \textsc{ Split Contraction}). Furthermore, we show that, assuming \textsf{ Gap-ETH}, there is no $\left(\frac{5}{4}-\delta \right)$-\FPT-approximation algorithm for \textsc{Split Contraction}. Here, $\epsilon, \delta>0$ are fixed constants. $(3)$ \textsc{Chordal Contraction} is known to be \WTH. We complement this result by observing that the existing \textsf{W[2]-hardness} reduction can be adapted to show that, assuming \FPT $\neq$ \textsf{W[1]}, there is no $F(k)$-\FPT-approximation algorithm for \textsc{Chordal Contraction}. Here, $F(k)$ is an arbitrary function depending on $k$ alone.

==> CHANGELOG <==
LIPICS Style - CHANGELOG

* 10/12/2018 LIPIcs-v2019 v2.0
** New Features
*** support of metadata in PDF file (e.g. author, title, keywords) 
*** revised displaying of author-related funding acknowledgements (now displayed as part of the funding block instead of footnotes)
*** added support for cleveref package (new document option 'cleveref')
*** added support for using autoref for theorem-like environments (new document option 'autoref')
*** added new environment claim and claimproof to realize sub-proofs
*** added new environment proposition
** Bugfixes
*** fixed problems with theorem-like environments when using cleveref and autoref (see new features above)
*** switched several URL from http to https
*** fixed problems with using of ACM 2012 classification (deactivated subjclass and revised support of ccsdesc macro)
** Minor changes
*** moved ORCID symbol behind author name (according https://orcid.org/content/journal-display-guidelines)
*** added separator \and to split several affiliations
*** added warnings when package 'enumitem' or 'paralist' are loaded; they manipulate the pre-defined enumeration styles and are partly incompatible
*** preloaded package 'microtype' in style
*** revised spacings/font sizes for top matter

* 09/04/2018 LIPIcs-v2018 v1.5
** Bugfixes
*** Fixed problem with page style in case of many authors
*** Fixed aggregation of authors for ToC file

* 15/03/2018 LIPIcs-v2018 v1.4
** Bugfixes
*** Fixed enumerations
*** Fixed aggregation of authors for ToC file

* 26/02/2018 LIPIcs-v2018 v1.3
** Bugfixes
*** Fixed \hideLIPIcs
*** Fixed enumerations
*** Fixed typo
** Revised display of ORCIDs following recommendation by ORCID

* 06/02/2018 LIPIcs-v2018 v1.2
** Release of LIPIcs-v2018
*** revised author macro \author{name}{affil}{email}{orcid}{funding} 
*** added support for ORCIDs
*** switched to ACM 2012 classification system
*** added new macros for extended metadata \category, \relatedversion, \supplement, \funding, \acknowledgements
*** added warnings for missing mandatory metadata
*** added preconfigured enumeration styles based on the enumerate package
*** added option \hideLIPIcs to hide all LIPIcs related information
*** added support for line numbers
** Bugfixes
*** fixed copyright line
*** added warning when using outdated subfig package due to incompatibilities in preloaded subcaption package
*** fixed bug when using MnSymbol package
*** fixed bug in numbering in theorem-like environments used in appendix
*** fixed problems in ToC file


==> preamblenew.tex <==
\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}


\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}
\usepackage{xcolor}
\usepackage{mdframed}


\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{amssymb,amsmath,mathrsfs}
\usepackage{soul}
\usepackage{mathtools}
\usepackage{framed}
\usepackage{xspace}

\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{red}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{green}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{blue}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}

\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amstext}
\usepackage{graphicx,tikz}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}
\usepackage{todonotes}
%\usepackage[linesnumbered, boxed, algosection,noline]{algorithm2e}

\usepackage{graphics}
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
%\usepackage{todonotes}

\newcommand{\OO}{\mathcal{O}}
\newcommand{\cO}{\mathcal{O}}

\usepackage{vmargin}
\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{redrule}{Reduction Rule}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{reduction}{Reduction Rule}[section]
\newtheorem{conjecture}{Conjecture}[section]

\mathchardef\myhyphen="2D
 
\newcommand{\defparproblem}[4]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
}\vspace{1mm}}

\newcommand{\defproblem}[3]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #3
  \end{minipage}
}\vspace{1mm}}

\usepackage{booktabs}
\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hyperfigures
                 ]{hyperref}

% general
\newcommand{\yes}{\textsf{Yes}\xspace}
\newcommand{\no}{\textsf{No}\xspace}
\newcommand{\yesinstance}{\yes-instance\xspace}
\newcommand{\noinstance}{\no-instance\xspace}
\newcommand{\tw}{\mathtt{tw}\xspace}
\newcommand{\NP}{\textsf{NP}\xspace}
\newcommand{\coNP}{\textsf{co-NP}\xspace}
\newcommand{\FPT}{\textsf{FPT}\xspace}
\newcommand{\XP}{\text{XP}\xspace}
\newcommand{\WO}{\textsf{W[1]}\xspace}
\newcommand{\WOH}{\textsf{W[1]}-hard\xspace}
\newcommand{\WOC}{\textsf{W[1]}-complete\xspace}
\newcommand{\WTH}{\textsf{W[2]}-hard\xspace}
\newcommand{\WTC}{\textsf{W[2]}-complete\xspace}
\newcommand{\NPH}{\textsf{NP}-hard\xspace}
\newcommand{\NPC}{\textsf{NP}-complete\xspace}
\newcommand{\paraH}{\textsf{para-NP}-hard}
\newcommand{\ETH}{\textsf{ETH}\xspace}
\newcommand{\SSE}{\textsf{SSE}\xspace}
\newcommand{\SETH}{\textsf{SETH}\xspace}
\newcommand{\nil}{\ensuremath{\mathtt{nil}}}
\newcommand{\opt}{\textsf{OPT}\xspace}
\newcommand{\prup}{1-\frac{1}{n^{26}}\xspace}
\newcommand{\pru}{\frac{1}{n^{26}}\xspace}

\newcommand{\supp}{\ensuremath{\mathtt{supp}}}
\newcommand{\coeff}{\ensuremath{\mathtt{coeff}}}
\newcommand{\MulLin}{\ensuremath{\mathtt{MulLin}}}

%specific to paper 
\newcommand{\mkk}{{\sc Min $k$-Cut}\xspace}
\newcommand{\cc}{\textsf{cc}\xspace}
\newcommand{\chd}{\textsf{children}\xspace}
\newcommand{\Pot}{\Phi}
%\newcommand{\adh}{\sigma}
\newcommand{\adh}{A}
\newcommand{\wh}[1]{\widehat{#1}}


%% Saket added 

\newcommand{\SpC}{\textsc{SpC}}
\newcommand{\SplitC}{\textsc{SplitC}}
\newcommand{\chc}{\textsc{Chordal Contraction}}
\newcommand{\al}{\alpha}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\B}{\ensuremath{\mathcal B}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\ClC}{\textsc{ClC}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\F}{\ensuremath{\mathbb F}}
\newcommand{\calH}{{\mathcal H}}
\renewcommand{\L}{\ensuremath{\mathcal{L}}}
\newcommand{\calO}{\ensuremath{{\mathcal O}}}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\Oh}{\mathcal{O}}
\newcommand{\OPT}{\textsc{OPT}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\Q}{\ensuremath{\mathcal{Q}}}
\newcommand{\sStar}{\mathcal{S}^{\star}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\T}{\ensuremath{\mathbb T}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\bbT}{\mathbb{T}_{\ell}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calZ}{\mathcal{Z}}


\newcommand{\POLY}{\textsf{poly}}
\newcommand{\Complete}{\textsf{Complete}}
%\newcommand{\FPT}{\textsf{FPT}}
\newcommand{\NPH}{\textsf{NP-Hard}}
\newcommand{\WH}{\textsf{W[1]-Hard}}
\newcommand{\WTH}{\textsf{W[2]-Hard}}
\newcommand{\ETH}{\textsf{ETH}}
\newcommand{\Woc}{\textsf{W[1]}-Complete}
\newcommand{\CONP}{\textsf{coNP}}
\newcommand{\CONPpoly}{\textsf{coNP/poly}}
\newcommand{\CONPH}{\textsf{coNP}-hard}
\newcommand{\CONPC}{\textsf{coNP}-complete}
\newcommand{\NPComplete}{\textsf{NP-Complete}}
\newcommand{\Hard}{\textsf{Hard}}
\newcommand{\NPpoly}{\textsf{NP/poly}}
\newcommand{\coNPpoly}{\textsf{coNP/poly}}


